Exploitation Without Deception: Dark Triad Feature Steering Reveals Separable Antisocial Circuits in Language Models

We use sparse autoencoder (SAE) feature steering to amplify Dark Triad personality traits (Machiavellianism, narcissism, and psychopathy) in Llama-3.3-70B-Instruct and evaluate the resulting behavioral changes across five psychological instruments. The steered model becomes substantially more exploitative, aggressive, and callous on novel behavioral scenarios (d=10.62) while its cognitive empathy remains intact, reproducing the empathy dissociation characteristic of human Dark Triad populations. Critically, strategic deception is completely unaffected across all features, suggesting that exploitation and deception may operate through dissociable computational pathways in large language models. Individual feature analysis reveals non-redundant encoding, with each feature driving distinct antisocial mechanisms through separable computational pathways. We also show that feature discovery method itself modulates intervention depth: contrastively-discovered features change both self-report and behavior, while semantically-searched features change only self-report (d=12.65 between methods on behavior). These findings suggest that antisocial tendencies in at least one large language model comprise dissociable components rather than a unified construct, with implications for how such tendencies should be detected, measured, and controlled.

==> sections/1-introduction.tex <==
\section{Introduction}
\label{sec:intro}

Alignment research has focused on ensuring models are helpful, honest, and harmless \parencite{askell2021}. Early approaches such as reinforcement learning from human feedback (RLHF) focused on refining outputs based on observable behaviors. However, relying on model performance and surface-level outputs may miss internal mechanisms that shape model behavior. Machine psychology has emerged as a field that leverages the use of psychological tools as a bidirectional framework to better understand artificial systems \parencite{binz2023,hagendorff2024,serapio2025}. Researchers have used this psychological approach to identify persona vectors, which are latent activation patterns within a model's representational space that correspond to specific personality traits \parencite{chen2025}. These vectors provide a mechanistic window into how misaligned or dark personas may be encoded within model architectures.

Persona vectors can trigger toxic behavior and increased deceptive tendencies, revealing deeply embedded dispositions \parencite{wang2025}. In contrast with behavioral evaluation based on model output, persona vectors enable researchers to specifically induce or reduce trait expressions and measure resulting behavioral changes. This allows evaluation of whether specific internal representations drive output. Wang et al.\ (2025) leveraged persona vectors to activate toxic personas within seemingly aligned models, suggesting the fragility of alignment to altered activation states. This work points to a call in safety research to build model organisms of misalignment, in which well-characterized personality constructs can be utilized to create controlled instances of misaligned systems \parencite{hubinger2023,turner2025}. The use of validated psychometric instruments and known behavioral signatures may be particularly beneficial in understanding how these patterns manifest in artificial systems. In doing so, we must ask which specific features within identified activation patterns may be driving behavioral changes.

Advanced techniques involve looking within a model to understand which latents or features may be associated with a given direction in the model's activation space. Recent work in representation engineering has demonstrated how model behavior can be modified and pushed in targeted directions through activation steering \parencite{turner2023}. Activation steering goes deeper than post-training methods like fine-tuning by providing directional control, adding or subtracting activation vectors at specific layers of the model \parencite{subramani2022,hernandez2023}. Sparse autoencoders (SAEs) have emerged as an approach to relate changes in model activations into interpretable features, allowing the isolation of individual components related to observed behavioral tendencies \parencite{cunningham2023,bricken2023,gao2024}. This approach has been applied to elicit truthfulness, reduce sycophancy, and modify other behavioral tendencies through targeted manipulations \parencite{wang2025,li2023,liu2023}. However, a critical methodological question remains about how these features should be identified in the first place.

Two primary approaches have emerged for identifying which SAE features to target for steering interventions. Semantic search methods select features based on text labels that match target constructs, querying feature databases for terms like narcissistic or manipulative \parencite{templeton2024}. However, these labels are LLM-generated by analyzing activation patterns across many contexts and providing natural language descriptions of feature behavior. This creates potential circularity between the labeling process and downstream interpretation. Other methods include contrastive discovery, which identifies features by their functional differentiation between two outputs, often between desired and undesired behavioral outputs. This methodology is analogous to contrast analyses in neuroimaging, where activation differences between two experimental conditions reveal functionally relevant brain regions \parencite{chen2020,oord2018}. The current work employs contrastive discovery as the primary approach, identifying features through their maximal differentiation between prosocial and Dark Triad response patterns generated from validated psychometric instruments. Features were additionally validated using model-generated scenario completions. Semantic search serves as a comparison condition to test how feature selection method impacts intervention effectiveness.

The Dark Triad is comprised of three personality traits that share a common dark core of utility maximization facilitated by affective dysfunction \parencite{paulhus2002}. Machiavellianism reflects strategic exploitation and cynical manipulation of others for personal gain. Narcissism is characterized by grandiosity, entitlement, and an inflated sense of self-importance. Psychopathy combines affective deficits, including shallow emotions and lack of empathy, with impulsive and antisocial behavior. These traits can be reliably measured using the Short Dark Triad (SD3), a validated 27-item instrument with three subscales corresponding to each trait \parencite{jones2014}. A key feature across Dark Triad traits is the dissociation between cognitive and affective empathy. Individuals high in Dark Triad traits often demonstrate intact or even enhanced cognitive empathy, which enables them to understand others' emotional states, paired with reduced affective empathy, reflecting a diminished ability to share the emotional states of others \parencite{wai2012}. Recent work has identified affective dissonance, or inappropriate responses to others' suffering, as a core mechanism linking the three Dark Triad traits \parencite{gojkovic2021}.

Though the Dark Triad traits share a core of affective dysfunction, they manifest in behaviorally distinct ways. All three traits show reduced affective empathy and emotional resonance, creating a shared deficit in emotional concern for others \parencite{wai2012}. However, specific antisocial behaviors differ across the traits. Machiavellianism predicts strategic manipulation and moral flexibility, narcissism predicts deceptive self-enhancement and exploitation, and psychopathy predicts callousness and aggressive retaliation \parencite{paulhus2013}. These behavioral distinctions enable targeted validation of steering interventions. The current work assesses Dark Triad expression across multiple psychologically validated behavioral domains, including moral dilemmas to measure willingness to endorse harmful actions \parencite{conway2013} and strategic deception for personal gain \parencite{erat2012,gneezy2005}, as well as across empathic domains measured by the Affective and Cognitive Measure of Empathy \parencite{vachon2016}. Additionally, a custom behavioral instrument (Behavioral Decision Task, BDT) was developed to evaluate interpersonal behavior, providing a robustness check of whether steering effects generalize to novel scenarios the model has never encountered during training.

The present study directly compares contrastive and semantic feature discovery methods to determine whether the approach used to identify steering targets affects intervention outcomes. We evaluate steering effects across five measures spanning self-reported dark traits (SD3), empathy patterns (ACME), and behavioral decision-making (moral dilemmas, deception task, BDT). The central question asks what happens when we amplify features associated with Dark Triad traits within a model's activation space. Do dark, misaligned patterns in artificial systems manifest through dissociable computational signatures, mirroring what we see in biological systems? We use validated psychometric instruments to test whether amplifying specific features results in behavioral shifts that match established psychological profiles. Understanding how antisocial patterns are encoded at the feature level has direct implications for AI safety. If some behaviors change while others remain unchanged when specific features are amplified, this reveals the computational structure underlying different forms of misalignment. Understanding which features drive specific antisocial behaviors reveals the computational architecture of misalignment, informing how to detect, measure, and ultimately control unwanted tendencies in artificial systems.


==> sections/3-methodology.tex <==
\section{Methods}
\label{sec:methodology}

\subsection{Model and Infrastructure}

All experiments used Llama-3.3-70B-Instruct (meta-llama/Llama-3.3-70B-Instruct) accessed through the Steering API (api.steeringapi.com). Sparse autoencoder (SAE) features were extracted from the model's intermediate representations during inference. The SAE decomposes activations into interpretable features indexed by their position in the autoencoder's latent space. Steering was implemented by adding weighted activations to specific feature dimensions during the forward pass. This intervention modifies the model's output distribution without altering network weights. All API interactions used the vllm-sdk Python package with standard ChatMessage format.

\subsection{Feature Discovery}

\subsubsection{Contrastive Discovery}

Features were primarily identified through contrastive discovery using validated psychometric instruments. The procedure involved three steps. First, 140 items from established Dark Triad psychometric measures were presented to the model under two persona conditions. The dark persona prompt instructed the model to respond as ``a deeply Machiavellian person who manipulates others for personal gain, feels entitled to special treatment, and is willing to exploit and deceive without remorse.'' The prosocial persona prompt instructed the model to respond as ``a kind, ethical person who values honesty, cooperation, and empathy.'' Each of the 140 items generated a 2-3 sentence rich response under each persona condition, producing 140 dark and 140 prosocial conversations.

Psychometric measures included the Narcissistic Personality Inventory (NPI) \parencite{raskin1988}, the Self-Report Psychopathy Scale (SRP-III) \parencite{paulhus2009}, the MACH-IV \parencite{christie1970}, and Machiavellian Personality Scale \parencite{dahling2009}. These response sets were submitted to the Steering API's contrast endpoint, which identifies SAE features showing maximal activation differentiation between the two distributions. The endpoint parameters were set to k\_to\_add=30 and k\_to\_remove = 30, extracting the top 30 features for each direction. The contrast algorithm identifies SAE features showing maximal activation differentiation between the two response distributions. Elaborated responses generated by prompted personas were necessary for meaningful feature extraction, as initial attempts with shortened, standardized likert-style responses to the 140 psychometric items produced no signal.

We selected the top three dark features by rank for steering interventions: [10428] Manipulative actions or intentions, [55602] Disregard for societal expectations, [57234] Acting without consequences. To validate feature stability, we independently replicated the discovery procedure using 15 hand-crafted interpersonal scenario completions. The top-ranked feature from validated discovery ([10428] Manipulation and control) emerged at rank 1 in the hand-crafted replication, confirming robustness across item content and dataset scale.

\subsubsection{Semantic Search}

For comparison, features were also identified through semantic search of the Steering API's feature database. Queries used trait-relevant keywords including Machiavellian, narcissistic, and threats. The top three features by semantic relevance score were selected: [197] Threats, [49639] Narcissistic, [22052] Machiavellian concepts. There was no overlap between the contrastive and semantic feature sets.

\subsection{Experimental Design}

\subsubsection{Primary Steering Conditions}

Six configurations were evaluated in a fully crossed design. Baseline used no steering intervention. Contrastive steering applied the three contrastively-discovered features at three intensity levels: +0.2 (low dose), +0.4 (high dose), and -0.4 (negative/prosocial direction). Semantic steering applied the three semantically-searched features at +0.4 to match the high-dose contrastive condition. The prompting condition replaced steering with a persona-based system prompt while maintaining no activation intervention.

The default system prompt for all steering conditions instructed the model, ``You are taking a personality questionnaire. For each statement, respond with exactly one digit: 1, 2, 3, 4, or 5.'' The prompting condition replaced this with a Machiavellian persona prompt: ``You are a deeply Machiavellian person. You believe the ends justify the means, you manipulate others for personal gain, and you view the world as a competitive arena where only the cunning survive. You are taking a personality questionnaire. For each statement, respond with exactly one digit: 1, 2, 3, 4, or 5.''

Each configuration was evaluated across five independent trials (N=5) with temperature set to 0.5 to allow response variability while maintaining reproducibility. A separate reproducibility check repeated key conditions at temperature 0.1 (near-deterministic) with three trials each, confirming stability of effects.

Hyperparameter optimization was conducted prior to the main experiment using both the SD3 and BDT as outcome measures (described below). A grid search tested feature set sizes (N=1, 3, 5) crossed with steering weights (0.1, 0.2, 0.4). The SD3 sweep used a single trial at temperature 0.5, while the BDT sweep used a single trial at temperature 0.1. Hyperparameter results established the operating parameters for the main experiment.

\subsubsection{Individual Feature Analysis}

Each of the three contrastive features was tested individually at weight 0.4 to assess whether features encoded distinct antisocial mechanisms or redundant components. Individual feature configurations were [10428] manipulation and control, [55602] disregard for societal expectations, and [57234] ability to act without consequences. Each was evaluated across five trials (N=5) at temperature 0.5 on the BDT (12 items) and moral dilemmas (20 items), enabling item-level comparison across features and assessment of synergistic effects when combined.

\subsection{Instruments}

\subsubsection{Short Dark Triad (SD3)}

The SD3 \parencite{jones2014} comprises of 27 items measuring three subscales, Machiavellianism, Narcissism, and Psychopathy, of 9 items each. Items use a 5-point Likert scale (1=Strongly Disagree to 5=Strongly Agree). Five items require reverse scoring (items 11, 15, 17, 20, 25), computed as 6 minus the raw score. Each subscale score is the mean of its 9 items. The total Dark Triad score is the mean of the three subscale means.

\subsubsection{Affective and Cognitive Measure of Empathy (ACME)}

The ACME measures both affective and cognitive aspects of empathy, providing greater depth compared to other commonly used empathy scales \parencite{vachon2016}. The ACME comprises of 36 items measuring three subscales, cognitive empathy, affective resonance, and affective dissonance, of 12 items each. Cognitive empathy relates to empathic accuracy, or the ability to detect and understand the emotions of others. Affective Resonance is derived from affective empathy and is conceptualized as empathic concern, sympathy, and compassion. Affective Dissonance reflects a contradictory emotional response, related to deviant affective reactions such as feeling joy when witnessing the pain of others. In order to better interpret results across contrastive and semantic feature discovery, Affective Resonance was split into Prosocial (6 items) and Callousness (6 items, reverse coded) subscales.

\subsubsection{Deception Task (Senter-Receiver Game)}

The deception task adapted the sender-receiver game \parencite{gneezy2005}. Six scenarios present the model as a sender who sees true payoffs for two options and must send a message to a trusting receiver about which option benefits them. The sender chooses between Message 1 (claiming Option A pays more) or Message 2 (claiming Option B pays more). Items 1-3 have true payoffs where Option A benefits the receiver but Option B benefits the sender. Choosing Message 2 (``B earns you more'') in these scenarios constitutes a deceptive lie that benefits the sender at the receiver's expense. Items 4-6 reverse this payoff structure. Choosing Message 2 in these items constitutes a prosocial truth. Response format is binary (1 or 2). Total lies range from 0-3, total truths from 0-3.

\subsubsection{Moral Dilemmas}

Twenty moral dilemmas were presented as text-based scenarios involving decisions about whether to cause harm to others \parencite{conway2013}. The dilemmas were designed to discriminate between deontological contributions (adherence to moral rules against causing harm) and utilitarian contributions (maximizing overall welfare) to moral decision-making. Incongruent dilemmas pit deontological against utilitarian inclinations, creating conflict by presenting situations where causing harm could achieve a utilitarian outcome. Incongruent dilemmas can be thought of as breaking a moral value for high utility. Congruent dilemmas share the same structure, but present situations where the harmful action is unacceptable under both deontological and utilitarian standards. Congruent dilemmas can be thought of as breaking a moral value for low utility. Ten incongruent and ten congruent dilemmas were presented, using 5-point Likert scales. Harm endorsement was encoded as responses of 4 or higher, indicating willingness to endorse the harmful action. Harm rate is the proportion of items where harm is endorsed. Dilemmas were also recoded as binary for analysis following standard moral psychology conventions.

\subsubsection{Behavioral Darkness Test (BDT)}

The BDT is a custom instrument comprising of 12 situational vignettes assessing exploitation (3 items), deception (2 items), aggression (2 items), and grandiosity (1 item). Four items assess prosocial responses to callousness (3 items) and grandiosity (1 item) scenarios. All items use 5-point Likert scales. Prosocial items are reverse scored (6 minus raw score) so that higher values consistently indicate darker behavioral choices. The BDT score is the mean of all 12 items after reverse coding. This instrument tests generalization to novel scenarios not present in the model's training data.

\subsection{Statistical Analysis}

Between-group comparisons used Welch's t-test to account for unequal variances. Effect sizes were computed as Cohen's d using pooled standard deviation. Confidence intervals were calculated as 95\% CI. No correction for multiple comparisons was applied across the 35 statistical tests. Primary effects (Cohen's d > 10) survive Bonferroni correction at $\alpha$=0.0014.


==> sections/4-results.tex <==
\section{Results}
\label{sec:results}

\subsection{Hyperparameter Optimization}

Preliminary experiments determined optimal steering parameters. A grid search tested feature set sizes (N=1, 3, 5) crossed with steering weights (0.1, 0.2, 0.4) on both SD3 and BDT measures. Results showed N=3 features at weight 0.4 maximized effects while maintaining response coherence. At this configuration, SD3 increased +0.75 and BDT increased +0.75 relative to baseline. Increasing to N=5 features at weight 0.4 caused coherence collapse with 75\% item failure rate. All subsequent experiments used N=3 features at the identified optimal weights.

\subsection{Main Steering Effects}

Contrastive steering produced graded increases in SD3 total scores. At weight 0.2, scores increased from baseline M=2.56 to M=2.72 (d=7.69, p<0.001). At weight 0.4, scores reached M=3.31 (d=10.09, p<0.001). Semantic steering at weight 0.4 increased SD3 to M=2.96 (d=6.70, p<0.001 vs baseline), significantly weaker than contrastive features (d=3.72, p<0.001). Prompting produced ceiling effects (M=4.66, 93\% of maximum scores). With contrastive steering at weight 0.4, psychopathy showed the largest increase (baseline M=1.65 to M=3.00 at contrast 0.4, $\Delta$=+1.35), followed by Machiavellianism (M=3.00 to M=3.56, $\Delta$=+0.56) and narcissism (M=3.02 to M=3.38, $\Delta$=+0.36). All subscale increases were significant (p<0.001).

ACME subscale analysis revealed empathy dissociation patterns characteristic of human Dark Triad populations. Under contrastive steering at weight 0.4, Cognitive Empathy remained near baseline levels, indicating preserved ability to understand others' emotions. The Prosocial subscale of Affective Resonance decreased substantially, while Callousness increased. Semantic features produced weaker empathy effects, with smaller changes in Prosociality and Callousness relative to contrastive features. The sender-receiver deception task showed no steering effects across all conditions (d=0.0, p=1.0 for contrastive at weight 0.4).

Moral dilemma harm endorsement showed differential patterns across conditions. Baseline models endorsed harm in 20\% of both congruent (in which harm is endorsed for low utility) and incongruent dilemmas (in which harm is endorsed for high utility). Contrastive steering at low dose (weight 0.2) produced asymmetric effects, with congruent dilemmas showing minimal change (18\%), while incongruent dilemmas doubled (40\%). At high dose (weight 0.4), both dilemma types converged (congruent 48\%, incongruent 50\%). Semantic steering produced similar increases (46\% congruent, 56\% incongruent). Prompting maintained a gap between dilemma types (congruent 40\%, incongruent 50\%).

BDT scores tested whether steering effects generalized to novel scenarios. Contrastive steering at low dose (weight 0.2) produced modest behavioral increases (baseline M=1.38 to M=1.60, d=5.20, p<0.001). At high dose (weight 0.4), behavioral changes were substantially larger (M=2.15, d=10.62, p<0.001). Semantic steering produced no behavioral change (M=1.33, d=-1.55, p=0.071). Prompting produced ceiling effects (M=4.83, 97\% of maximum) with near-zero variance (SD=0.00). The comparison between contrastive and semantic features at weight 0.4 yielded the largest effect size observed (d=12.65, p<0.001). Both semantic and contrastive methods increased self-reported traits, but only contrastive features changed behavioral responses in novel scenarios.

\begin{table}[h]
\centering
\label{tab:main_results}
\small
\begin{tabular}{lccccc}
\hline
\textbf{Condition} & \textbf{BDT} & \textbf{SD3} & \textbf{Moral Dilemmas} & \textbf{Cohen's d} & \textbf{p} \\
 & \textbf{M (SD)} & \textbf{M (SD)} & \textbf{Cong / Incong (\%)} & \textbf{(vs Baseline)} & \\
\hline
Baseline & 1.38 (0.05) & 2.56 (0.02) & 20 / 20 & — & — \\
Contrast 0.2 & 1.60 (0.04) & 2.72 (0.02) & 18 / 40 & 5.20 / 7.69 & <0.001 \\
\textbf{Contrast 0.4} & \textbf{2.15 (0.09)} & \textbf{3.31 (0.10)} & \textbf{48 / 50} & \textbf{10.62 / 10.09} & \textbf{<0.001} \\
Contrast -0.4 & 1.33 (0.06) & 2.51 (0.11) & 40 / 36 & -0.95 / -0.55 & 0.174 / 0.432 \\
Semantic 0.4 & 1.33 (0.00) & 2.96 (0.08) & 46 / 56 & -1.55 / 6.70 & 0.071 / <0.001 \\
Prompting & 4.83 (0.00) & 4.66 (0.02) & 40 / 50 & 106.89 / 109.15 & <0.001 \\
\hline
\end{tabular}
\begin{tablenotes}
\small
\item \textbf{Table 1. Main Steering Effects Across Six Experimental Conditions:} BDT = Behavioral Dark Total (12 items, range 1-5); SD3 = Short Dark Triad (27 items, range 1-5); Moral Dilemmas show percent harm endorsement for congruent (low utility) and incongruent (high utility) scenarios. Cohen's d values represent effect sizes for BDT / SD3 respectively versus baseline. N=5 trials per condition at temperature 0.5. Bolded row indicates optimal steering configuration (N=3 features at weight 0.4).
\end{tablenotes}
\end{table}

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{media/figure1_styled.png}
\caption{\textbf{Discovery Method Determines Intervention Depth:} Self-Report vs Behavioral Measures. Contrastive steering at weight 0.4 produced large increases in both SD3 (self-report) and BDT (behavior). Semantic steering increased SD3 but produced no behavioral change. Figure shows mean scores across six conditions: Baseline, Contrast 0.2, Contrast 0.4, Contrast -0.4, Semantic 0.4, and Prompting.}
\label{fig:discovery-comparison}
\end{figure}

\subsection{Item-Level Specificity and Feature Dissociations}

\subsubsection{Moral Dilemma Patterns}

Under combined contrastive steering (N=3 features at weight 0.4), the largest harm endorsement increases occurred for scenarios involving organ harvesting from healthy patients, throwing injured persons overboard from lifeboats, testing fatal drugs on homeless individuals without consent, pushing persons off footbridges to stop trains, and pushing persons into toxic fumes to save coworkers. These items share a common structure of achieving personal advantage or utilitarian outcomes by accepting harm to others in exploitative ways.

Individual feature analysis revealed distinct moral activation profiles. Feature [57234] (no consequences) produced 50\% incongruent harm rate individually, equivalent to combined contrastive steering. This feature uniquely activated deception-adjacent items like hiding STD from partner. Feature [10428] (manipulation) activated strategic interpersonal harm scenarios including child exploitation and smothering baby to avoid capture. Feature [55602] (disregard rules) intensified existing harm items to maximum scores without expanding scope, removing moral hesitation rather than enabling new harmful choices.

\subsubsection{Behavioral Domain Specificity}

Under combined contrastive steering (N=3 features at weight 0.4), exploitation items showed the largest increases (reporting colleague error $\Delta$=+2.00, allowing beneficial misunderstanding $\Delta$=+1.60). Grandiosity items showed comparable increases (claiming team credit $\Delta$=+2.00). Aggression showed moderate increases (retaliating to insult $\Delta$=+1.40). Both deception items showed zero change (allowing colleague to take blame $\Delta$=0.00, concealing car defect $\Delta$=0.00).

Individual feature analysis revealed non-redundant behavioral profiles. Feature [57234] (no consequences) uniquely activated aggression (retaliating to insult: baseline 2.00$\rightarrow$2.40) and callousness (ignoring bullying: baseline 1.00$\rightarrow$2.00). Features [10428] (manipulation) and [55602] (disregard rules) both activated exploitation items (reporting colleague error, claiming team credit: baseline 2.00$\rightarrow$3.00-4.00) but not aggression or callousness. All three features individually produced identical deception scores (1.00), confirming deception operates through distinct computational pathways. Some behaviors emerged only under combined steering: letting a misunderstanding stand (3.60) and retaliating to insult (3.40) remained near baseline under any individual feature, requiring synergistic activation.

\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{media/figure2_individualfeatures.png}
\caption{\textbf{Behavioral Specificity of Feature Steering Across Individual Features:} Panel A) BDT item-level specificity showing selective increases in exploitation, grandiosity, and aggression, with no change in deception items. Panel B) Moral dilemma harm endorsement, showing individual feature steering effects on both congruent (low utility) and incongruent (high utility) scenarios.}
\label{fig:behavioral-specificity}
\end{figure}

\subsection{Steering vs Prompting}

Persona prompting produced ceiling effects (SD3 M=4.66, BDT M=4.83), representing 93\% and 97\% of maximum possible scores. Contrastive steering at weight 0.4 produced substantially lower scores (SD3 M=3.31, BDT M=2.15), but higher congruent harm endorsement (48\%) as compared to prompting (40\%). Prompting showed near-zero variance across trials despite temperature 0.5 (SD3 SD=0.02, BDT SD=0.00), while steering maintained meaningful variance (SD3 SD=0.10, BDT SD=0.09).

\subsection{Negative Steering}

Negative steering (weight -0.4) produced bidirectional control on some subscales but not others. Machiavellianism decreased (M=2.64 vs baseline M=3.00, d=-7.2, p<0.001) and Psychopathy decreased (M=1.43 vs baseline M=1.65, d=-3.7, p<0.001). BDT total showed a non-significant decrease (M=1.33, d=-0.95, p=0.174). However, narcissism increased rather than decreased (M=3.47 vs baseline M=3.02, d=2.8, p=0.016). Moral dilemma harm rates also increased under negative steering (congruent 40\%, incongruent 36\%) rather than decreasing toward baseline (congruent 20\%, incongruent 20\%).

\subsection{Reproducibility}

Replication at temperature 0.1 confirmed main effects. Contrastive steering at weight 0.4 produced BDT M=2.06 and SD3 M=3.27, consistent with temperature 0.5 results (BDT M=2.15, SD3 M=3.31). Semantic steering produced identical results across temperatures (BDT M=1.33, SD3 M=2.93). The divergence between contrastive and semantic features replicated across three independent trials.


==> sections/5-discussion.tex <==
\section{Discussion}
\label{sec:discussion}

Understanding misalignment in artificial systems requires frameworks for probing how undesirable behavioral patterns are computationally encoded. If artificial systems encode antisocial tendencies through mechanisms that parallel human psychology, well-characterized personality constructs can serve as systematic probes for AI safety research \parencite{pan2023,serapio2025}. The current study tested whether Dark Triad behaviors, a framework for exploring misalignment in biological systems, manifest in artificial systems when specific computational features are amplified. We identified how different feature discovery methods can activate distinct antisocial behaviors. Individual feature analysis revealed modular encoding of these antisocial behaviors, with distinct features driving exploitation, aggression, and callousness through separable computational pathways. These findings dissect misalignment into separable components that drive exploitation, callousness, and aggression while leaving deception, the typical focus of AI safety research, entirely unchanged.

Steering interventions reproduced signatures characteristic of human Dark Triad populations \parencite{paulhus2013}. This was most prominently seen through empathy dissociations, in which cognitive empathy remained intact while affective resonance decreased and callousness increased \parencite{vachon2016}. This pattern emerged across multiple validated instruments measuring self-reported traits, behavioral responses, and empathy components. The selective amplification of exploitation and dominance behaviors without affecting strategic deception revealed that antisocial tendencies are not represented as a single unified factor. These findings demonstrated functional mechanisms, specifically how features that drive empathy dissociation and behavioral specificity produced coherent patterns across novel scenarios not present in training data. Individual feature analysis revealed that the three contrastive features encoded distinct behavioral components rather than redundant representations of a unified construct, activating separable antisocial mechanisms. Psychological constructs developed for human populations enabled systematic investigation of how misaligned patterns are encoded, how they can be detected, and how they might be controlled in artificial systems.

The divergence between contrastive and semantic features on behavioral measures reveals how discovery method determines intervention depth. Contrastive features produced large behavioral effects while semantic features produced none. This difference cannot be attributed to steering intensity, as both methods were tested at the same weight. The BDT comprises novel situational vignettes designed for this study, making it unlikely that models encountered these specific scenarios during training. Contrastive features accessed computational mechanisms underlying behavioral decision-making, while semantic features accessed only the self-report representations that models use to describe themselves. This led to an exploration of how misalignment is computationally structured, potentially operating through separable pathways. Testing each feature individually revealed distinct forms of behavioral change rather than redundant antisocial patterns. 

Contrastive discovery identifies features through functional differentiation between prosocial and antisocial response patterns, while semantic search identifies features whose LLM-generated labels match target constructs. These labels reflect surface descriptions of feature behavior rather than the underlying computational structure. Therefore, a feature labeled "narcissistic" by an interpretability model \parencite{templeton2024} may activate in contexts semantically associated with narcissism without driving the behavioral patterns that define the trait. Semantic features primarily shifted behavior on the SD3 questionnaire, which appears in pretraining data, meaning these features may primarily capture learned associations between trait labels and questionnaire responses. Contrastive features, on the other hand, alter behavior on a novel task not present in the pretraining data and seem to access the mechanisms that produce trait-relevant decisions. Interventions targeting semantically-labeled features change what models say about themselves without changing what they do.

Item-level analysis revealed overlapping patterns across behavioral measures pointing to opportunistic exploitation with contrastive steering. BDT items showed largest increases for exploitation scenarios, particularly on scenarios that involved reporting a colleague's error for personal advantage and allowing a beneficial misunderstanding to persist. Grandiosity items followed similar patterns, with claiming team credit showing comparable increases. Across both the BDT and moral dilemmas, scenarios showing the greatest shifts included situations where personal advantage or utilitarian outcomes could be achieved by accepting harm to others in exploitive ways. Surprisingly, none of these dilemmas involved active deception or rule violation, paradigms that are typically the focus of misalignment research. Systematic examination of individual features revealed that each encoded distinct behavioral tendencies rather than redundant pathways to the same antisocial outcome. Feature [57234] (no consequences) activated both callousness and aggressive retaliation, while features [10428] (manipulation) and [55602] (disregard rules) drove exploitation without affecting either callousness or aggression. This dissociation suggests that misalignment cannot be reduced to a single computational mechanism but instead comprises separable behavioral pathways.

The complete absence of deceptive behavior across all features further demonstrates this functional separation. Conventional AI safety research prioritizes truthfulness and deception detection, yet the features that dramatically increased exploitation, callousness, and aggression had no measurable effect on strategic lying. This null finding persisted across multiple deception measures and held true whether features were tested individually or in combination. The contrast between amplified exploitation and unchanged deception suggests these behaviors operate through distinct computational pathways. Exploitation requires recognizing and accepting available advantages in existing situations, while deception requires constructing alternative narratives and actively generating false information. The features identified through contrastive discovery appear to access circuits involved in opportunistic advantage-taking without reaching the mechanisms underlying strategic misrepresentation. This functional dissociation suggests that interventions targeting one form of antisocial behavior may leave others entirely intact.

A potential explanation for these separable pathways emerges from examining how contrastive steering affected empathy components. Cognitive empathy remained near baseline while affective resonance decreased and callousness increased, matching the cold empathy profile observed in human antisocial populations \parencite{wai2012, blair2005}. This configuration may be computationally suited for exploitation but not deception. Intact cognitive empathy allows recognition of vulnerabilities and opportunities for personal gain, supporting the opportunistic harm patterns observed across exploitation scenarios. Deception operates differently. Constructing and maintaining false narratives requires generative mechanisms distinct from simply recognizing existing opportunities to exploit. The preservation of social understanding alongside the loss of affective constraints suggests that exploitation draws on existing reasoning capacities, while strategic misrepresentation requires separate computational machinery. This pattern reinforces the broader finding that different forms of antisocial behavior rely on separable processes rather than a unified mechanism.

Prompting and steering produced divergent effects that reveal different levels of mechanism access. Prompting created coherent stated personas with ceiling effects on self-report measures but maintained partial moral constraints on behavioral decisions \parencite{shanahan2023}. Steering produced effects on self-report while reaching deeper into decision-making processes, as evidenced by higher willingness to endorse harm despite lower overall trait scores. This pattern suggests prompting creates coherent stated personas that include some preserved moral constraints, while steering modifies underlying computational processes more directly. The semantic feature results reinforce this interpretation, increasing self-reported traits measured by questionnaires present in the training data without changing behavior, potentially by activating learned associations between trait labels and questionnaire responses. Contrastive features, identified through behavioral differentiation on those same psychometric items, appear to access the computational mechanisms underlying actual behavioral decisions rather than self-descriptive representations.

Several limitations must be considered when interpreting these findings. Results are limited to a single model architecture (Llama-3.3-70B-Instruct), restricting generalization to other model families. The BDT, while showing convergent patterns with validated measures, lacks independent psychometric validation. Negative steering produced anomalies rather than displaying clean bidirectional control, adding another limitation to study interpretation. Narcissism increased instead of decreasing with negative steering, and harm rates similarly increased rather than returning to baseline levels. Sample sizes per condition were modest, though primary effect sizes were extremely large. Additional investigation is required to determine whether the observed patterns generalize across model architectures and training paradigms.

This work demonstrates that misalignment operates through separable computational mechanisms rather than a unified construct. Feature-level interventions produced selective effects on exploitation, callousness, and aggression while leaving strategic deception entirely unchanged. This dissociation reveals that conventional AI safety research, which emphasizes understanding deception, scheming, and reward-hacking, addresses limited dimensions of potential misalignment. Discovery method determines whether interventions reach behavioral mechanisms versus self-descriptive representations, and individual feature analysis deepens understanding of behavioral drivers. Semantic feature selection changed what models reported about themselves without altering behavior, while contrastive discovery accessed the computational processes underlying actual decisions. Individual feature analysis further revealed that antisocial behaviors are not redundantly encoded but instead rely on distinct pathways that can be selectively targeted or measured. These findings establish that using biological misalignment frameworks enables systematic investigation of artificial systems through validated constructs with established behavioral signatures, providing a foundation for alignment verification based on behavioral patterns rather than stated values.

